ReCode: Updating Code API Knowledge with Reinforcement Learning

Large Language Models (LLMs) exhibit remarkable code generation capabilities but falter when adapting to frequent updates in external library APIs. This critical limitation, stemming from reliance on outdated API knowledge from their training data, even with access to current documentation, impedes reliable code generation in dynamic environments. To tackle this issue, we propose ReCode (rule-based Reinforcement learning for Code Update), a novel framework that mimics human programmer adaptation to API changes. Specifically, we construct a dataset of approximately 2,000 data entries to train the LLMs to perform version migration based on updated information. Then, we introduce a modified string similarity metric for code evaluation as the reward for reinforcement learning. Our experiments demonstrate that ReCode substantially boosts LLMs' code generation performance in dynamic API scenarios, especially on the unseen CodeUpdateArena task. Crucially, compared to supervised fine-tuning, ReCode has less impact on LLMs' general code generation abilities. We apply ReCode on various LLMs and reinforcement learning algorithms (GRPO and DAPO), all achieving consistent improvements. Notably, after training, Qwen2.5-Coder-7B outperforms that of the 32B parameter code instruction-tuned model and the reasoning model with the same architecture. Code is available at https://github.com/zjunlp/ReCode.

==> mul-update.tex <==
\begin{prompt}[title={\thetcbcounter {} Error Case}]

\promptsubsection{System}\\
You are a helpful code assistant. 
You first think about the reasoning process in the mind and then provide a Python solution to a problem in a real-world scenario.

\promptsubsection{User}\\
Update Note:

There's an recent update to a function math.degrees -- The math.degrees function is updated to enable conversion from radians and another unit through an additional parameter.

The function now has a new function signature -- math.degrees(x, input\_unit='radian').

Here is a detailed documentation about the update:

<doc>

Scenario: You are working on a scientific computing project, where angle calculations are a crucial part. However, not all your data sources provide angles in the same measurement units, some are providing angle values in radians and others in gradians. You are aiming to standardize all angles to degrees for improved interoperability.

Problem: Given an angle value and the unit it's provided in (either 'radian' or 'gradian'), write a function to convert it into degrees.

Solution signature: function convert\_angle\_to\_degrees(angle: float, unit: str) -> float:

Show your work in <think> </think> tags.
And return the final code in <answer> </answer>, the code within <answer></answer> should be enclosed in ```python ``` tags.

\promptsubsection{Assistant}\\
Let me solve this step by step. \\
<think>

1. First, I need to understand how to convert radians to degrees. The formula is degrees = radians * (180 / $\pi$).

2. Next, I need to understand how to convert gradians to degrees. The formula is \textcolor{red}{degrees = gradians * (90 / 200)}.

3. Now, I need to create a function that takes two parameters: the angle value and its unit ('radian' or 'gradian').

4. Inside the function, I'll check the unit parameter. If it's 'radian', I'll use the radians to degrees formula. If it's 'gradian', I'll use the gradians to degrees formula.

5. If the unit parameter is neither 'radian' nor 'gradian', I'll raise a ValueError with the appropriate message.

6. Finally, I'll return the converted angle value.

</think>

<answer>
\begin{lstlisting}[language={python}]
import math

def convert_angle_to_degrees(
    angle: float, unit: str
) -> float:
    if unit == 'radian':
        return angle * (180 / math.pi)
    elif unit == 'gradian':
        return angle * (90 / 200)
    else:
        raise ValueError('input_unit \
        should be either radian \
        or gradian')
\end{lstlisting}
</answer>

\end{prompt}
